Guarding Serverless Applications with SecLambda

As an emerging application paradigm, serverless computing attracts attention from more and more attackers. Unfortunately, security tools for conventional applications cannot be easily ported to serverless, and existing serverless security solutions are inadequate. In this paper, we present \emph{SecLambda}, an extensible security framework that leverages local function state and global application state to perform sophisticated security tasks to protect an application. We show how SecLambda can be used to achieve control flow integrity, credential protection, and rate limiting in serverless applications. We evaluate the performance overhead and security of SecLambda using realistic open-source applications, and our results suggest that SecLambda can mitigate several attacks while introducing relatively low performance overhead.

==> background.tex <==
\section{Background}

\tnote{This sections eems like a bit of an orphan. Can we integrate the cnotent
into flow of next section somewhere?} 



==> eval2.tex <==
\section{Real-world serverless applications}\label{sec:eval}
\begin{figure*}[t]
\begin{center}
\includegraphics[width=0.8\linewidth]{figure/app_examples}
\end{center}
\caption{Flow graphs of the target applications. Rectangles, rounded rectangles
and dotted lines represent function, third-party services, and implicit flows, respectively. 
The entry functions that accept user requests are highlighted. }
\label{fig:app_flow}
\end{figure*}

\begin{table}[t]
\center
\footnotesize
\begin{tabular}{|l|r|r|r|r|}
\hline
 & \multicolumn{1}{l|}{\textbf{LOC}} & \multicolumn{1}{l|}{\textbf{\#Func}} & \multicolumn{1}{l|}{\textbf{\#Lib}} & \multicolumn{1}{l|}{\textbf{Language}} \\ \hline \hline
\helloapp & 5,127 & 12 & 158 & Node.js \\ \hline
\codeapp & 2068 & 9 & 112 & Node.js \\ \hline
\mapapp & 7,47 & 3 & 1 & Python \\ \hline
\end{tabular}
\caption{An overview of the lines of code, number of functions and third-party modules, and 
the languages of the target applications.}
\label{tab:app_overview}
\end{table}


We evaluate the efficiency of flow graph functions with real-world serverless applications.
We choose for our evaluation three open-source serverless applications for AWS Lambda: \helloapp~\cite{hello}, 
\codeapp~\cite{code}, and \mapapp~\cite{map}. \helloapp, a retail platform developed by Nordstrom, 
is the most sophisticated open-source serverless application we have known. 
\codeapp is an application from AWS for automatically updating the deployment 
script of software after its source code or configuration has been modified. 
\mapapp is a serverless-based MapReduce framework. 
The three applications demonstrate the use of different 
features of serverless: \helloapp takes advantage of the event sourcing mechanism 
and AWS Step Functions to pass messages among functions and invoke function automatically,  
\codeapp purely leverages AWS Step Functions to automatically execute functions in order, 
and \mapapp relies on the auto-scaling feature to run functions in parallel. 
\tabref{tab:app_overview} and \figref{fig:app_flow} show an overview of the three applications 
and flow graphs. 


\subsection{Evaluation setup}\label{sec:eval:setup}
In AWS Lambda, we cannot modify the provided function runtime. 
As a workaround, we modify the Python and Node.js modules that 
are used by our target applications for sending requests, and instrument the 
functions to use the modified modules. As for evaluation, 
we only need to modify the ssl module~(\texttt{ssl.py}) in Python, 
and the aws-sdk modules~(only \texttt{aws-sdk/libs/http/node.js}) 
in Node.js. Since there are no local file operations in the applications, we do not modify 
any modules related to file operations. We instrument every function to launch a guard asynchronously in a 
background process and wait for 1 second to ensure that the guard is fully initialized, 
before processing events. Without modifying the infrastructures of AWS, 
\sysname cannot achieve full functionality. Nevertheless, AWS provides a 
realistic environment for more accurately evaluating the accuracy of 
auto-generated flow policies. 

The controller ran 
on a m5.large VM in the AWS us-east-1 region, and all the experiments were 
conducted in the same region unless otherwise stated. 

\subsection{Microbenchmark}
\bheading{Policy checking overhead.}
%
When enforcing the local flow graph, the guard only needs to maintain one pointer 
that points to the current flow. The time of moving the pointer is negligible, 
so is the policy checking time. In the latency test, we let the guard perform 1,000 iterations of 
policy checking. The average overhead (across 500 invocations of the test function)
for 1,000 policy checks is \SI{89.1}{\micro\second} (SD=\SI{43.7}{\micro\second}) and \SI{73.2}{\micro\second} (SD=\SI{44.2}{\micro\second}) 
when the function memory sizes are 128\,MB and 2,048\,MB respectively. 
The maximum overhead in any settings is less than \SI{220}{\micro\second}. We believe 1,000  
is a reasonable large size for local flow graph, so 
for ordinarily applications the policy checking overhead is sufficiently low.  
Overall, operations (policy checking, message manipulation, etc.) 
other than communications only account for a negligible portion of the overhead introduced by \sysname.


\bheading{Controller communication overhead.}
%
We further measured the round-trip latency between the guard and the controller 
under different message sizes and function memory sizes. We measured the latency
100 times for a given setting. The results are shown in \tabref{tab:ctr_rtt}. 
The round-trip latency not only determines guard startup time but also affects 
function runtime, because the guard will communicate with the controller if the function 
receives messages from third-party services. Besides, the 
efficiency of the rate limiting security function is also affected by this latency: 
the longer time it takes the guard to receive the \texttt{STOP} message 
back from the controller, the more requests that can be sent before being stopped. Considering that 
the messages exchanged between the guard and the controller are less than 1\,KB 
except during guard startup, and in one function execution the guard  
communicates with the controller synchronously at most once, the overhead 
introduced by guard-controller communications is around just 6\,ms   
for functions of large memory sizes (i.e., 1,024\,MB).


\begin{table}[t]
\center
\footnotesize
\renewcommand\tabcolsep{2pt}
\begin{tabular}{|l|r|r|r|r|}
\hline
 & \multicolumn{1}{c|}{\textbf{128}} & \multicolumn{1}{c|}{\textbf{512}} & \multicolumn{1}{c|}{\textbf{1024}} & \multicolumn{1}{c|}{\textbf{2048}} \\ \hline
 \hline
\textbf{1\,KB} & 65.6 (13.3) & 11.6 (6.1) & 6.5 (2.3) & 5.1 (0.7) \\ \hline
\textbf{10\,KB} & 69.8 (15.0) & 11.3 (5.5) & 7.4 (2.1) & 5.2 (0.6) \\ \hline
\textbf{1\,MB} & 945.2 (143.1) & 222.4 (11.9) & 100.6 (5.3) & 61.7 (2.0) \\ \hline
\end{tabular}
\caption{The average controller communication latencies and standard derivations (in ms) across 
100 rounds under different message sizes and memory sizes.}
\label{tab:ctr_rtt}
\end{table}


\subsection{Flow graph generation}\label{sec:eval:graph}
We started with writing a minimum set of test cases that cover all 
the execution paths of the target applications.
Based on their documentation and state machines (provided by Step Functions), 
we created 4, 3, and 1 test cases for 
\helloapp, \codeapp, and \mapapp, respectively. Several functions are triggered only  
when there are errors during request processing. In one round of test, 
we run all the test cases once with random user input. In \helloapp, user 
requests are for creating products, to register photographers, and to query products, so 
we generate random product/photographer information and query strings. \codeapp 
will be triggered automatically when there are changes to the monitored repository, 
and we add 1--5 random files (1\,KB) in the monitored repository. For \mapapp, 
the job is fixed as word count, and user requests specify the dataset and number 
of files to be processed. We randomly choose one dataset from the \emph{text/tiny/rankings} and 
\emph{text/tiny/uservisits} datasets 
in the Big Data Benchmark from AMPLab~\cite{bigdata}, and process 1--9 files in a 
request~(the datasets only have 9 files). All the other settings remain default. 

We obey the limits (request rate, input size, etc.) of all the APIs when constructing the requests, 
because violating these limits will not generate any new paths, but may cause 
Step Functions to be stuck for minutes, which unnecessarily prolongs the experiment time.   

We ran the test for 1,000 rounds. After analyzing the collected traces, we find  
a clear gap between expected flows and real flows from a function. 
Only two functions are associated with consistent flows in any test, 
while neither function actually makes any outgoing connections. For 
the rest of the functions, we collected varied numbers of unique traces. Note that 
the extra flows do not necessary affect the global flow graph (i.e., 
no new execution paths).    

We identify three unexpected causes for the varied flows:

\begin{newenum}
\item \emph{API library implementation}: 
API libraries may add randomness to endpoints' URLs. 
For instance, the AWS API for sending data to AWS Codepipeline (used by 
the \texttt{CreateChangeSet} function in \codeapp) will automatically append a short,  
random string to the URL of AWS Codepipeline to distinguish different requests.  

\item \emph{Service configuration}: Server-side configuration such as HTTP redirection 
will introduce extra flows that cannot be inferred from code. 

\item \emph{Network failures or other unknown service behaviors}: In some cases, the 
function will retry a request if the request failed due to unstable network condition 
or received duplicated messages from services.

\end{newenum}

Other than these, flows may vary according to user input: In \mapapp, the \texttt{Mapper} function 
will download data from S3 multiple times depending on the size of user data. Similarly, 
the \texttt{Coordinator} function will create different number of reducers based on user data. 
Besides, the exact URLs for the files in S3 will also vary.  

The final local graphs contain only 1--9 nodes (excluding the begin and end nodes). 
The median size (i.e., number of nodes) of the local graphs for \helloapp, \codeapp, 
and \mapapp are 3, 2, and 7, respectively. The global graphs generated 
are consistent with the state machines in Step Functions or the expected 
graph got from manual inspection. Maintaining these graphs in memory incurs negligible 
memory overhead. 



\begin{figure}[t]
\begin{center}
\input{figure/graph_error.tex}
\end{center}
\caption{Errors when using the traces collected from different numbers of rounds  
for building flow graphs.}
\label{fig:flowerror}
\end{figure}

Intuitively, more rounds of tests will produce more accurate flow graphs.
Based on the collected traces, we further estimate when using the traces from the first $n$ rounds 
to build flow graphs, the number of rounds the guards will block flows and cause function failures. 
As shown in \figref{fig:flowerror}, the traces from one round of test can cover 
the requests in about 40\%, 80\%, and 65\% of rounds, and no errors when using 583, 7, and 463 rounds of traces    
in \helloapp, \codeapp, and \mapapp respectively. See \secref{sec:eval:security} for more 
discussions of the security implications of our graph generation approach.   


% Most of the functions 
% can be modeled efficiently with less than 100 rounds of traces except for 
% two ``bottlenecks'':the \texttt{Report} function in \hellomapp and the \texttt{Reducer} function in \mapapp.

% \subsection{Flow Association Efficiency}\label{sec:eval:infer}
% Our flow tracking function does rely the lazy message association heuristics \secref{sec:app:flowtracking} 
% but we still want to estimate to which extent the heuristics can accurately 
% associate messages to requests in cloud environments and provide insights for future similar research.
% We used \helloapp to evaluate the heuristics. We sent 
% $k$~($k=2, 4, 6, 8, 10$) requests to \helloapp with a waiting time of $t$~($t = 0, 0.5, 1, 2, 3$) 
% seconds between requests, where $t = 0$ means the requests are sent concurrently. 
% We first focused on the \texttt{Assign} and \texttt{SendAssignment} (or simply \texttt{Send}) 
% functions (see \figref{fig:app_flow}). The \texttt{Send} function will be 
% invoked by Step Functions only if \texttt{Assign} returns expected results. 
% We recored the time \texttt{Assign} sent responses to Step Functions,  
% the time \texttt{Send} were invoked, and the request ID (created by Step Functions) 
% in the events received by the functions. Ideally, \texttt{Send} should receive 
% the events in the same order as \texttt{Assign} processes the events. 
% For a given $k, t$ combination, we sent 100 requests and examined how many times 
% \texttt{Send} received out-of-order events. We conducted the same experiment for the 
% \texttt{Processor} and \texttt{Catalog} functions, who have an implicit flow through Kinesis. 
% As we can see from \figref{fig:acc}, when the waiting time between two requests 
% increase from 0 (concurrently) to 3 seconds, the probability of receiving events in order 
% increases from 80\% to 95\%. And the probability drops greatly as the service processes 
% more requests in a shorter time period. The results suggest for infrequent 
% and non-concurrent requests, our lazy method may be helpful for distinguishing 
% the messages belonging to different requests. But overall, because of 
% cloud services' unpredictable performance, timing-based heuristics may  
% not be the optimal way for such task under realistic workloads.

% \begin{figure}[t]
% \begin{center}
% \input{figure/acc.tex}
% \end{center}
% \caption{The probability of receiving events in order under various number 
% of requests. The series indicate different waiting time between two requests, while 0 
% means all requests are sent concurrently. }
% \label{fig:acc}
% \end{figure}




% \begin{table}[t]
% \center
% \footnotesize
% \renewcommand\tabcolsep{2pt}
% \begin{tabular}{|l|r|r|r|r|}
% \hline
%  & \multicolumn{1}{c|}{\textbf{128}} & \multicolumn{1}{c|}{\textbf{512}} & \multicolumn{1}{c|}{\textbf{1024}} & \multicolumn{1}{c|}{\textbf{2048}} \\ \hline
%  \hline
% \textbf{1\,KB} & 65.6 (13.3) & 11.6 (6.1) & 6.5 (2.3) & 5.1 (0.7) \\ \hline
% \textbf{10\,KB} & 69.8 (15.0) & 11.3 (5.5) & 7.4 (2.1) & 5.2 (0.6) \\ \hline
% \textbf{1\,MB} & 945.2 (143.1) & 222.4 (11.9) & 100.6 (5.3) & 61.7 (2.0) \\ \hline
% \end{tabular}
% \caption{The average controller communication latencies and standard derivations (in ms) across 
% 100 rounds under different message sizes and memory sizes.}
% \label{tab:ctr_rtt}
% \end{table}


 
\subsection{Security analysis}\label{sec:eval:security}

The flow graphs generated by our flow tracking function represent relatively 
tight security policies. Even with a slight difference between the expected URL and its URL, 
a flow will be considered as invalid and be blocked. The generated flow graphs 
do not contain cycles or loops, and any given path in a graph represents 
a legitimate order of flows or function executions. Therefore, the 
flow tracking function can prevent an attacker from generating arbitrary flows from the 
compromised function, and reduces the risk of data leakage via restricting the ways 
for the attacker to externalize data. The loop counter associated with a node indicates 
how many times the flow can occur in a normal function execution. 
If it occurs more than the expected times, the flow will be blocked to prevent potential attacks.   

The attacker may try to bypass some functions (e.g., authentication) to 
invoke a target function directly. For instance, the attacker invokes the \texttt{CreateChangeSet} 
function in \codeapp directly to modify source code of a software. Though 
the resulting flows are legitimate, the flow tracking function may still block such attempts: 
if the requests come from invalid sources or 
do not carry correct tags, or the preceding function of the target function 
is not at a correct state, the execution will 
be blocked. Basically, we do not allow an application execution to begin from 
the middle of an execution path. The attacker may try to exploit the race condition 
between function executions to therefore perform a type of flow injection attacks. For example, 
the attacker leverages some vulnerabilities in Step Functions to execute  
\texttt{CreateChangeSet} just before a normal execution of \texttt{CreateChangeSet} begins. 
In this case, the controller will assume the attacker-launched execution is legitimate, 
but can still detect anomalies (See \secref{sec:flowtracking:global} \emph{Concurrent requests}).        

As we discussed in \secref{sec:eval:graph}, static analysis 
will not be sufficient for understanding the flows generated under realistic workloads. 
Using dynamic analysis, security depends on the quality of test cases. 
The flow graphs will be more accurate with test cases that can cover more paths.
However, we may still encounter uncovered cases during normal application executions, 
which could cause execution failures. One possible option is to switch 
from fail closed to fail open, i.e., the system records suspicious flows 
rather than block~them.

The nodes with the LCP URLs 
allow the flows whose destination URLs share the same prefix, which may cause security issues. 
However, without them the resulting graphs could be too restrictive  
so that they cannot handle change in user input. 
For example in \mapapp, without using LCP URLs, the flows for 
fetching different files (who have the same prefix and are in the format of 
``prefix0000'',...,``prefix000n'') will produce distinguish nodes and any future 
requests that are not for fetching these files will be blocked. We believe 
manual inspection of flow graphs is a reasonable way to solve this issue. 
The tenant can adjust the threshold being used to produce the optimal flow graphs 
and examine whether the nodes with the LCP URLs are appropriate.   

% The flow graphs have two special types of URLs: LCP and wildcard. 
% We do not have the wildcard URL in the flow graphs for the tested applications, 
% but this could be useful for some applications. Since the nodes with the wildcard URLs allow 
% arbitrary flows, security cannot be guaranteed. Similarly, 

The flow tracking function cannot prevent attacks that exploits   
both legitimate function and application control flows, and data-related attacks (e.g., 
modify the data sent by a compromised function). However, it is feasible to extend our 
framework and develop more sophisticated security functions to achieve 
finer-grained information flow control for serverless. 


% The credentials management function should be used with flow tracking function. 
% An attacker may manipulate messages to change where the token placeholders are placed. 
% But by replacing the sensitive data from response messages,    


% When we replace the dummy token 
% We show two ways for the guard to add credentials in the requests. The first 
% way is to reconstruct the message, and the second way is to locate the 
% placeholder (i.e., the random string is a placeholder for the access token) 
% for a given credential and replace the placeholder with the credential. The second 
% method might be vulnerable to credential leakage if the attacker manipulates 
% the message payload to inject placeholders and the API server 
% echoes back the invalid message. However, we have not seen any popular APIs behaving in 
% this way so far so this method should be sufficient in most cases. The first method 
% can avoid the aforementioned attacks since the tenant basically reconstructs the 
% message body, though MAY require more efforts on understanding message format and 
% introduce extra (neglectable) delay





==> eval_bk.tex <==
\section{Evaluation}\label{sec:eval}


We consider two settings in our evaluation. A local testbed is set up for  
evaluating the performance overhead of runsec due to the fact that we cannot modify 
existing serverless platforms. Open-source serverless applications cannot directly 
run in the local testbed because they may require   


To evaluate the efficiency of the flow tracking function, 
we 

\begin{figure*}[t]
\begin{center}
\includegraphics[width=0.8\linewidth]{figure/app_examples}
\end{center}
\caption{Flow graphs of the target applications. Rectangles, rounded rectangles
and dotted lines represent function, third-party services, and implicit flows, respectively. 
The entry functions that accept user requests are highlighted. }
\label{fig:app_flow}
\end{figure*}

\begin{table}[t]
\center
\footnotesize
\begin{tabular}{|l|r|r|r|r|}
\hline
 & \multicolumn{1}{l|}{\textbf{LOC}} & \multicolumn{1}{l|}{\textbf{\#Func}} & \multicolumn{1}{l|}{\textbf{\#Lib}} & \multicolumn{1}{l|}{\textbf{Language}} \\ \hline \hline
\helloapp & 5,127 & 12 & 158 & Node.js \\ \hline
\codeapp & 2068 & 9 & 112 & Node.js \\ \hline
\mapapp & 7,47 & 3 & 1 & Python \\ \hline
\end{tabular}
\caption{An overview of the lines of code, number of functions and third-party modules, and 
the languages of the target applications.}
\label{tab:app_overview}
\end{table}



We choose for our evaluation three open-source serverless applications for AWS Lambda: \helloapp~\cite{hello}, 
\codeapp~\cite{code}, and \mapapp~\cite{map}. \helloapp, a retail platform developed by Nordstrom, 
is the most sophisticated open-source serverless application we have known. 
\codeapp is an application from AWS for automatically updating the deployment 
script of software after its source code or configuration has been modified. 
\mapapp is a serverless-based MapReduce framework. 
The three applications demonstrate the use of different 
features of serverless: \helloapp takes advantage of the event sourcing mechanism 
and AWS Step Functions to pass messages among functions and invoke function automatically,  
\codeapp purely leverages AWS Step Functions to automatically execute functions in order, 
and \mapapp relies on the auto-scaling feature to run functions in parallel. 
\tabref{tab:app_overview} and \figref{fig:app_flow} show an overview of the three applications 
and flow graphs. 


\subsection{Evaluation setup}\label{sec:eval:setup}
In AWS Lambda, we cannot modify the provided function runtime. 
As a workaround, we modify the Python and Node.js modules that 
are used by our target applications for sending requests, and instrument the 
functions to use the modified modules. As for evaluation, 
we only need to modify the ssl module~(\texttt{ssl.py}) in Python, 
and the aws-sdk modules~(only \texttt{aws-sdk/libs/http/node.js}) 
in Node.js. Since there are no local file operations in the applications, we do not modify 
any modules related to file operations. 
Without modifying the infrastructures of AWS, \sysname cannot achieve full functionality. 
Nevertheless, AWS provides a realistic environment for more accurately 
evaluating the accuracy of auto-generated flow policy (graph) and \sysname overhead. 

We instrument every function to launch a guard asynchronously in a 
background process and wait for 1 second to ensure that the guard is fully initialized, 
before processing events.~(We later found that
the actual guard startup time is much lower. See \secref{sec:eval:overhead}.) 
We will take 1 second off when calculating function execution time. 
Note that on a serverless platform that supports \sysname the guard should be 
launched during instance startup, which is before running any function.

Lambda only sends HTTP request bodies to functions, 
so the guard cannot access connection information and HTTP header information, and 
is not able to infer the source of a given request. In the target applications, 
fortunately, the services being used will carry identity information in the 
messages~(for services that are able to serve as event source of functions),  
or we are able to add sender identity information in their messages. 
Without accessing headers, the guard also cannot manipulate tags. For the purpose of 
overhead evaluation, we still let the guard adds a tag to the HTTP header in 
a request sent from the function, and simulate the tag removal operation by 
removing the last field from the HTTP header in a response and putting 
that field back. 

We implemented a prototype of \sysname and the security functions in C/C++~(about 3\,K 
lines of code). Different components in \sysname use \emph{zeromq} for communication~\cite{zeromq}.   
We added 90 lines of code in total for modifying Python and Node.js modules.
In the evaluation, we only deploy the flow tracking function. The controller ran 
on a m5.large VM in the AWS us-east-1 region, and all the experiments were 
conducted in the same region unless otherwise stated. 

\subsection{Flow graph generation}\label{sec:eval:graph}
We started with writing a minimum set of test cases that cover all 
the execution paths of the target applications.
Based on their documentation and state machines (provided by Step Functions), 
we created 4, 3, and 1 test cases for 
\helloapp, \codeapp, and \mapapp, respectively. Several functions are triggered only  
when there are errors during request processing. In one round of test, 
we run all the test cases once with random user input. In \helloapp, user 
requests are for creating products, to register photographers, and to query products, so 
we generate random product/photographer information and query strings. \codeapp 
will be triggered automatically when there are changes to the monitored repository, 
and we add 1--5 random files (1\,KB) in the monitored repository. For \mapapp, 
the job is fixed as word count, and user requests specify the dataset and number 
of files to be processed. We randomly choose one dataset from the \emph{text/tiny/rankings} and 
\emph{text/tiny/uservisits} datasets 
in the Big Data Benchmark from AMPLab~\cite{bigdata}, and process 1--9 files in a 
request~(the datasets only have 9 files). All the other settings remain default. 

We obey the limits (request rate, input size, etc.) of all the APIs when constructing the requests, 
because violating these limits will not generate any new paths, but may cause 
Step Functions to be stuck for minutes, which unnecessarily prolongs the experiment time.   

We ran the test for 1,000 rounds. After analyzing the collected traces, we find  
a clear gap between expected flows and real flows from a function. 
Only two functions are associated with consistent flows in any test, 
while neither function actually makes any outgoing connections. For 
the rest of the functions, we collected varied numbers of unique traces. Note that 
the extra flows do not necessary affect the global flow graph (i.e., 
no new execution paths).    

We identify three unexpected causes for the varied flows:

\begin{newenum}
\item \emph{API library implementation}: 
API libraries may add randomness to endpoints' URLs. 
For instance, the AWS API for sending data to AWS Codepipeline (used by 
the \texttt{CreateChangeSet} function in \codeapp) will automatically append a short,  
random string to the URL of AWS Codepipeline to distinguish different requests.  

\item \emph{Service configuration}: Server-side configuration such as HTTP redirection 
will introduce extra flows that cannot be inferred from code. 

\item \emph{Network failures or other unknown service behaviors}: In some cases, the 
function will retry a request if the request failed due to unstable network condition 
or received duplicated messages from services.

\end{newenum}

Other than these, flows may vary according to user input: In \mapapp, the \texttt{Mapper} function 
will download data from S3 multiple times depending on the size of user data. Similarly, 
the \texttt{Coordinator} function will create different number of reducers based on user data. 
Besides, the exact URLs for the files in S3 will also vary.  

The final local graphs contain only 1--9 nodes (excluding the begin and end nodes). 
The median size (i.e., number of nodes) of the local graphs for \helloapp, \codeapp, 
and \mapapp are 3, 2, and 7, respectively. The global graphs generated 
are consistent with the state machines in Step Functions or the expected 
graph got from manual inspection. Maintaining these graphs in memory incurs negligible 
memory overhead. 



\begin{figure}[t]
\begin{center}
\input{figure/graph_error.tex}
\end{center}
\caption{Errors when using the traces collected from different numbers of rounds  
for building flow graphs.}
\label{fig:flowerror}
\end{figure}

Intuitively, more rounds of tests will produce more accurate flow graphs.
Based on the collected traces, we further estimate when using the traces from the first $n$ rounds 
to build flow graphs, the number of rounds the guards will block flows and cause function failures. 
As shown in \figref{fig:flowerror}, the traces from one round of test can cover 
the requests in about 40\%, 80\%, and 65\% of rounds, and no errors when using 583, 7, and 463 rounds of traces    
in \helloapp, \codeapp, and \mapapp respectively. See \secref{sec:eval:security} for more 
discussions of the security implications of our graph generation approach.   


% Most of the functions 
% can be modeled efficiently with less than 100 rounds of traces except for 
% two ``bottlenecks'':the \texttt{Report} function in \hellomapp and the \texttt{Reducer} function in \mapapp.

% \subsection{Flow Association Efficiency}\label{sec:eval:infer}
% Our flow tracking function does rely the lazy message association heuristics \secref{sec:app:flowtracking} 
% but we still want to estimate to which extent the heuristics can accurately 
% associate messages to requests in cloud environments and provide insights for future similar research.
% We used \helloapp to evaluate the heuristics. We sent 
% $k$~($k=2, 4, 6, 8, 10$) requests to \helloapp with a waiting time of $t$~($t = 0, 0.5, 1, 2, 3$) 
% seconds between requests, where $t = 0$ means the requests are sent concurrently. 
% We first focused on the \texttt{Assign} and \texttt{SendAssignment} (or simply \texttt{Send}) 
% functions (see \figref{fig:app_flow}). The \texttt{Send} function will be 
% invoked by Step Functions only if \texttt{Assign} returns expected results. 
% We recored the time \texttt{Assign} sent responses to Step Functions,  
% the time \texttt{Send} were invoked, and the request ID (created by Step Functions) 
% in the events received by the functions. Ideally, \texttt{Send} should receive 
% the events in the same order as \texttt{Assign} processes the events. 
% For a given $k, t$ combination, we sent 100 requests and examined how many times 
% \texttt{Send} received out-of-order events. We conducted the same experiment for the 
% \texttt{Processor} and \texttt{Catalog} functions, who have an implicit flow through Kinesis. 
% As we can see from \figref{fig:acc}, when the waiting time between two requests 
% increase from 0 (concurrently) to 3 seconds, the probability of receiving events in order 
% increases from 80\% to 95\%. And the probability drops greatly as the service processes 
% more requests in a shorter time period. The results suggest for infrequent 
% and non-concurrent requests, our lazy method may be helpful for distinguishing 
% the messages belonging to different requests. But overall, because of 
% cloud services' unpredictable performance, timing-based heuristics may  
% not be the optimal way for such task under realistic workloads.

% \begin{figure}[t]
% \begin{center}
% \input{figure/acc.tex}
% \end{center}
% \caption{The probability of receiving events in order under various number 
% of requests. The series indicate different waiting time between two requests, while 0 
% means all requests are sent concurrently. }
% \label{fig:acc}
% \end{figure}




\subsection{SecLambda overhead}\label{sec:eval:overhead}

\bheading{Guard communication overhead.}
%
We started with measuring overhead in a controlled environment. We set up 
a web server in the AWS us-east-1 region, and created a Python-based test function of 
$m$ MB memory to send HTTPs requests to fetch a 1\,KB file from the web server $n$ times. 
We created two different versions of the library for sending HTTPs requests: one communicates   
with the guard and one does not. 
In the experiment, we adjusted $m$ ($m$=128, 512, 1,024, 2,048) and $n$ ($n$ = 5, 10, 15, 20, 50, 100), 
and invoked the function 100 times for a given $m$ and $n$. In each invocation, 
the function will send $n$ requests twice, with and without guard being enabled, 
and report (1) the \emph{overhead}, which is the 
difference in the function runtimes for two rounds of requests,  
and (2) the \emph{guard round-trip latencies} of function-guard calls (i.e., the time elapsed 
between when the function sends a message to the guard and when it gets the decision from the guard). 
Note that we only created the function once 
so the function was running in the same function instance throughout the experiment. 
The guard is initialized with a dummy local flow graph that has one path with 1,000 nodes and each URL is 
a random string of 1,024 bytes. The guard checks all the nodes to emulate the policy lookup time.   

As expected, guard round-trip latency increases as function memory decreases. 
In Lambda, the CPU cycles assigned to a function instance are proportional to the function's 
allocated memory. We show the performance variance 
in function runtime without using \sysname in \figref{fig:guard_mem} (b) for reference. 
The median guard round-trip 
latency across all function-guard calls 
is 18.8 \,ms when $m$ = 128\,MB, and 0.48 \,ms when $m$ = 2,048\,MB. 
The variance of latency is high for the 128\,MB function, ranging from 0.41\,ms 
to 398\,ms. As shown in 
\figref{fig:guard_mem} (a), the latency becomes more stable as function memory increases. 


\begin{figure}[t]
\begin{center}
\input{figure/guard_mem_vs_rtt.tex}
\end{center}
\caption{CDFs of (a) guard round-trip latency 
and (b) function execution time (without guard) in milliseconds under different function memory sizes. 
The number of guard calls=10.}
\label{fig:guard_mem}
\end{figure}

% \begin{figure}[t]
% \begin{center}
% \input{figure/guard_mem_vs_tm.tex}
% \end{center}
% \caption{CDFs of function execution time (in ms, without guard) under different function memory sizes 
% when the number of HTTPs requests is 5.}
% \label{fig:guard_mem_tm}
% \end{figure}

\begin{figure}[t]
\begin{center}
\input{figure/guard_no_vs_rtt.tex}
\end{center}
\caption{The median of the per-guard-call overheads of functions (in ms) in different languages 
and memory sizes.}
\label{fig:guard_no_rtt}
\end{figure}

With guard being enabled, the function needs to communicates with the guard $2 \cdot n$ 
(when sending a HTTPs request and receiving a response) times for a given $n$. 
We observed that when $m$ is fixed, the overhead is almost proportional to $n$. 
The per-function-guard call overhead (the overhead under $n$ divided by $2 \cdot n$) 
is similar to the guard round-trip latency, as shown in \figref{fig:guard_no_rtt}.

We performed the same experiment for Node.js based functions. However, 
we cannot directly measure guard round-trip latency in Node.js functions. 
The reason is that Node.js sends requests asynchronously almost at the same time, 
and uses an event loop to handle responses. All the responses from the guard 
could be queued up and get processed one by one. Measuring the difference 
between request sending time and response receiving time will include 
the event loop waiting time. Therefore, we only focus on the per-guard-call overheads. 
As shown in \figref{fig:guard_no_rtt}, as the number of guard calls increases,  
the overhead introduced by event queuing increases. Also, function memory sizes 
have even more impact on Node.js function than on Python functions. 

\bheading{Controller communication overhead.}
%
We further measured the round-trip latency between the guard and the controller 
under different message sizes and function memory sizes. We measured the latency
100 times for a given setting. The results are shown in \tabref{tab:ctr_rtt}. 
The round-trip latency not only determines guard startup time but also affects 
function runtime, because the guard will communicate with the controller if the function 
receives messages from third-party services. Besides, the 
efficiency of the rate limiting security function is also affected by this latency: 
the longer time it takes the guard to receive the \texttt{STOP} message 
back from the controller, the more requests that can be sent before being stopped. Considering that 
the messages exchanged between the guard and the controller are less than 1\,KB 
except during guard startup, and in one function execution the guard  
communicates with the controller synchronously at most once, the overhead 
introduced by guard-controller communications is around just 6\,ms   
for functions of large memory sizes (i.e., 1,024\,MB).


\bheading{Policy checking overhead.}
%
When enforcing the local flow graph, the guard only needs to maintain one pointer 
that points to the current flow. The time of moving the pointer is negligible, 
so is the policy checking time. In the latency test, we let the guard perform 1,000 iterations of 
policy checking. The average overhead (across 500 invocations of the test function)
for 1,000 policy checks is \SI{89.1}{\micro\second} (SD=\SI{43.7}{\micro\second}) and \SI{73.2}{\micro\second} (SD=\SI{44.2}{\micro\second}) 
when the function memory sizes are 128\,MB and 2,048\,MB respectively. 
The maximum overhead in any settings is less than \SI{220}{\micro\second}. We believe 1,000  
is a reasonable large size for local flow graph, so 
for ordinarily applications the policy checking overhead is sufficiently low.  
Overall, operations (policy checking, message manipulation, etc.) 
other than communications only account for a negligible portion of the overhead introduced by \sysname.


\begin{table}[t]
\center
\footnotesize
\renewcommand\tabcolsep{2pt}
\begin{tabular}{|l|r|r|r|r|}
\hline
 & \multicolumn{1}{c|}{\textbf{128}} & \multicolumn{1}{c|}{\textbf{512}} & \multicolumn{1}{c|}{\textbf{1024}} & \multicolumn{1}{c|}{\textbf{2048}} \\ \hline
 \hline
\textbf{1\,KB} & 65.6 (13.3) & 11.6 (6.1) & 6.5 (2.3) & 5.1 (0.7) \\ \hline
\textbf{10\,KB} & 69.8 (15.0) & 11.3 (5.5) & 7.4 (2.1) & 5.2 (0.6) \\ \hline
\textbf{1\,MB} & 945.2 (143.1) & 222.4 (11.9) & 100.6 (5.3) & 61.7 (2.0) \\ \hline
\end{tabular}
\caption{The average controller communication latencies and standard derivations (in ms) across 
100 rounds under different message sizes and memory sizes.}
\label{tab:ctr_rtt}
\end{table}




% Controller message propagation delay is the time it takes for the guard to receive 
% the messages from the controller, which is the same as the one-way latency 
% from the controller to the guard. The message propagation delay not only affects  
% the guard startup time but also the efficiency of the rate limiting security function: 
% longer propagation delay means that more requests can be sent before being blocked.  
% We used the \texttt{Product} function (1\,GB memory)
% in \helloapp for testing, moved the controller to different regions, 
% and let the controller send messages of different sizes (1\,K, 1\,M, and 10\,M) 100 rounds. 
% The results are shown in \tabref{tab:polocy_prop}. Clearly, 
% the delay becomes longer as policy size and network distance increase. Since 
% the \texttt{STOP} message is less than 1\,KB, the guard will be able to stop 
% the requests that violate rate limits within about 12\,ms. 


\bheading{Real applications.}
%
We ran the minimal set of test cases for 100 rounds, and recorded 
the execution time of different functions. 
As shown in \tabref{tab:overhead}, the overhead is not directly related to  
the number of guard calls in \helloapp. The results are similar for \codeapp.
One reason is that Node.js sends requests asynchronously so the overhead cannot 
be simply estimated by the number of guard calls and per-guard-call overhead. 
In Python-based applications like \mapapp, the guard communication overhead is 
higher because the lower-bound on overhead is always at least the sum of per-guard-call overhead. 
Besides, AWS services might have unpredictable performance, affecting  
affect the function running time, even without guards. 
As in \tabref{tab:overhead}, the standard deviation of the running time of the \texttt{Receive} function (func8) in \helloapp can be 
up to 128\,ms because the function interacts with four services, and one of them, twilio, 
is outside of AWS. Lambda itself also suffers from unstable  
performance issues: resource contention and VM configuration significantly affect 
a function's performance. For instance, even running the guards 
without any function-to-guard communications may introduce 10\,ms to 25\,ms 
of overhead to the function runtime because the guard will compete for 
CPU resources. We suspect that such contention may cause high variance in the performance 
of CPU-intensive functions, such as the \texttt{Mapper} function~(func2) 
and the \texttt{Reducer} function~(func3) in \mapapp. And, the difference in the 
median execution times of the \texttt{Mapper} function in \mapapp  
in the instances running on different VMs can be up to 500\,ms 
(we invoked the function 50 times in each instance). 

To better understand the performance variance in the real cloud environment,  
we show the CDFs of the runtimes of the functions with the highest and second highest 
relative overhead, with and without \sysname, in the two applications in \figref{fig:reallatcdf}. 
The runtimes with and without \sysname actually lie within the same range except for a few outliers.  
And, since Lambda measures runtime in 100\,ms blocks, the overhead only costs 
an iota of extra money (\$0.000001667 per function).  
Overall, we believe the overhead introduced by \sysname is acceptable. 


\begin{table}[]
\center
\footnotesize
\renewcommand\tabcolsep{2pt}
\begin{tabular}{|l|r|r|r|r|}
\hline
\multicolumn{1}{|r|}{\textbf{Func}} & \textbf{W/ Guard (SD)} & \textbf{No Guard (SD)} & \textbf{Overhead (\%)} & \multicolumn{1}{r|}{\textbf{\#Min guard calls}} \\ \hline
1 & 25.2 (8.9) & 24.8 (24.9) & 0.3 (1.4) & 4 \\ \hline
2 & 28.7 (14.8) & 21.2 (9.8) & 7.6 (35.9) & 4 \\ \hline
3 & 29.1 (15.8) & 22.5 (9.5) & 6.7 (29.7) & 6 \\ \hline
4 & 38.0 (14.4) & 27.3 (15.5) & 10.7 (39.4) & 6 \\ \hline
5 & 47.0 (67.5) & 37.8 (83.8) & 9.1 (24.2)	 & 6 \\ \hline
6 & 67.4 (23.6) & 58.8 (13.5) & 8.6 (14.7) & 6 \\ \hline
7 & 151.8 (33.1) & 138.5 (32.5) & 13.4 (9.6)  & 6 \\ \hline
8 & 474.9 (69.6) & 461.8 (128.6) & 13.2 (2.8) & 8 \\ \hline
\hline
1 & 124.6 (22.8) & 111.4 (21.3) & 13.3 (11.9)  & 10 \\ \hline
2 & 1281.8 (91.3) & 1205.3 (60.6) & 76.6 (6.4) & 10 \\ \hline
3 & 1377.2 (293.5) & 1295.3 (113.7) & 81.9 (6.3) & 8 \\ \hline
\end{tabular}
\caption{An overview of the median runtime with/without guards, absolute and relative overhead 
(in ms), and number of guard calls of major functions in \helloapp (\textbf{upper}) and \mapapp (\textbf{lower}) 
across 100 rounds.}
\label{tab:overhead}
\end{table}



\begin{figure}[t]
\begin{center}
\includegraphics[width=0.75\linewidth]{figure/real_lat_cdf.eps}
\end{center}
\caption{CDFs of the runtimes of the functions with the highest and second highest 
relative overhead in \helloapp (\textbf{upper}) and \mapapp (\textbf{lower}).}
\label{fig:reallatcdf}
\end{figure}


% \subsection{Controller Message Propagation Delay}
% Controller message propagation delay is the time it takes for the guard to receive 
% the messages from the controller, which is the same as the one-way latency 
% from the controller to the guard. The message propagation delay not only affects  
% the guard startup time but also the efficiency of the rate limiting security function: 
% longer propagation delay means that more requests can be sent before being blocked.  

% We used the \texttt{Product} function (1\,GB memory)
% in \helloapp for testing, moved the controller to different regions, 
% and let the controller send messages of different sizes (1\,K, 1\,M, and 10\,M) 100 rounds. 
% The results are shown in \tabref{tab:polocy_prop}. Clearly, 
% the delay becomes longer as policy size and network distance increase. Since 
% the \texttt{STOP} message is less than 1\,KB, the guard will be able to stop 
% the requests that violate rate limits within about 12\,ms. 


% One benefit of using \sysname is that it can provide the same functionality 
% as AWS IAM role, while alleviates 
% the policy propagation delay issue in IAM. We conducted simple measurements 
% to demonstrate that IAM might introduce high policy propagation delay. 
% We set up an EC2 instance as the vantage point and a Lambda function that 
% we call \emph{caller function} in 
% the us-east-1 region. From the vantage point, we use AWS APIs to 
% attach/detach a policy that allows the function to access another function (\emph{callee function}) 
% or service (\emph{callee service}) to the role of the function. The task of 
% the caller function is just to invoke the callee functions or list the available 
% resources in the callee services. The callee function simply returns ``Hello World'', 
% and the callee service only has one resource so that the we can assume that the 
% callee can quickly process the requests from the caller function.  
% The callee functions are also in the us-east-1 region, and the services are S3, 
% DynamoDB, and CloudTrail. 

% After updating the policy, we keep invoking the caller function from the vantage 
% point until getting the expected result: the caller function should successfully get the response 
% from the callee after attaching the policy, or get ``access deny'' after detaching 
% the policy. As a baseline, the RTT latency for a request is less than 0.25\,ms 
% for any callees in any cases. We record the time (in seconds) it takes for the policy to be effective, 
% and conservatively evaluate the propagation delay by taking the greatest integer 
% less than the recored time as the delay. 
% We attached or detached the policy 100 times for each type of the callees, and 
% stopped invoking the caller function after 120 seconds after the policy update.
% For S3, DynamoDB, and CloudTrail, the median propagation delays 
% for attaching a policy were 0, 5, 0 seconds, and for detaching a policy 
% were 6, 0, 0 seconds. However, the longest delay for S3, DynamoDB, and CloudTrail 
% could be 10, 8, and more than 120 seconds, respectively.  
% The propagation delay in Lambda was higher: the minimum delay was 6 seconds, and 
% the median was about 110 seconds. We continued to invoke the caller function 
% after 120 seconds, and found the policy could eventually be effective within 300 seconds. 
% The is much worse than the worst case of \sysname (3.5\,s). 

\subsection{Security analysis}\label{sec:eval:security}

The flow graphs generated by our flow tracking function represent relatively 
tight security policies. Even with a slight difference between the expected URL and its URL, 
a flow will be considered as invalid and be blocked. The generated flow graphs 
do not contain cycles or loops, and any given path in a graph represents 
a legitimate order of flows or function executions. Therefore, the 
flow tracking function can prevent an attacker from generating arbitrary flows from the 
compromised function, and reduces the risk of data leakage via restricting the ways 
for the attacker to externalize data. The loop counter associated with a node indicates 
how many times the flow can occur in a normal function execution. 
If it occurs more than the expected times, the flow will be blocked to prevent potential attacks.   

The attacker may try to bypass some functions (e.g., authentication) to 
invoke a target function directly. For instance, the attacker invokes the \texttt{CreateChangeSet} 
function in \codeapp directly to modify source code of a software. Though 
the resulting flows are legitimate, the flow tracking function may still block such attempts: 
if the requests come from invalid sources or 
do not carry correct tags, or the preceding function of the target function 
is not at a correct state, the execution will 
be blocked. Basically, we do not allow an application execution to begin from 
the middle of an execution path. The attacker may try to exploit the race condition 
between function executions to therefore perform a type of flow injection attacks. For example, 
the attacker leverages some vulnerabilities in Step Functions to execute  
\texttt{CreateChangeSet} just before a normal execution of \texttt{CreateChangeSet} begins. 
In this case, the controller will assume the attacker-launched execution is legitimate, 
but can still detect anomalies (See \secref{sec:flowtracking:global} \emph{Concurrent requests}).        

As we discussed in \secref{sec:eval:graph}, static analysis 
will not be sufficient for understanding the flows generated under realistic workloads. 
Using dynamic analysis, security depends on the quality of test cases. 
The flow graphs will be more accurate with test cases that can cover more paths.
However, we may still encounter uncovered cases during normal application executions, 
which could cause execution failures. One possible option is to switch 
from fail closed to fail open, i.e., the system records suspicious flows 
rather than block~them.

The nodes with the LCP URLs 
allow the flows whose destination URLs share the same prefix, which may cause security issues. 
However, without them the resulting graphs could be too restrictive  
so that they cannot handle change in user input. 
For example in \mapapp, without using LCP URLs, the flows for 
fetching different files (who have the same prefix and are in the format of 
``prefix0000'',...,``prefix000n'') will produce distinguish nodes and any future 
requests that are not for fetching these files will be blocked. We believe 
manual inspection of flow graphs is a reasonable way to solve this issue. 
The tenant can adjust the threshold being used to produce the optimal flow graphs 
and examine whether the nodes with the LCP URLs are appropriate.   

% The flow graphs have two special types of URLs: LCP and wildcard. 
% We do not have the wildcard URL in the flow graphs for the tested applications, 
% but this could be useful for some applications. Since the nodes with the wildcard URLs allow 
% arbitrary flows, security cannot be guaranteed. Similarly, 

The flow tracking function cannot prevent attacks that exploits   
both legitimate function and application control flows, and data-related attacks (e.g., 
modify the data sent by a compromised function). However, it is feasible to extend our 
framework and develop more sophisticated security functions to achieve 
finer-grained information flow control for serverless. 


% The credentials management function should be used with flow tracking function. 
% An attacker may manipulate messages to change where the token placeholders are placed. 
% But by replacing the sensitive data from response messages,    


% When we replace the dummy token 
% We show two ways for the guard to add credentials in the requests. The first 
% way is to reconstruct the message, and the second way is to locate the 
% placeholder (i.e., the random string is a placeholder for the access token) 
% for a given credential and replace the placeholder with the credential. The second 
% method might be vulnerable to credential leakage if the attacker manipulates 
% the message payload to inject placeholders and the API server 
% echoes back the invalid message. However, we have not seen any popular APIs behaving in 
% this way so far so this method should be sufficient in most cases. The first method 
% can avoid the aforementioned attacks since the tenant basically reconstructs the 
% message body, though MAY require more efforts on understanding message format and 
% introduce extra (neglectable) delay





==> experiment.tex <==
\section{Evaluation}

\subsection{Performance evaluation in local testbed}
\liangw{will think about how to merge the local testbed and lambda results once we get all results.}
\bheading{Setup.}
%
We set up a single control plane Kubernetes cluster of five nodes, with each node running 
on an Intel(R) Xeon(R) CPU E5-2640 v4 @ 2.40GHz and 64GB of RAM machine.  
Each machine is connected to a star topology LAN network with a speed of 25\,Gbps. 
The \sysname controller runs on a separate identical node outside the LAN but on the same datacenter. 

\bheading{Guard-checking overhead.}
%
We create a Python-based  
test function to send 1000 HTTP identical GET request to a web server in the same cluster. 
We run the function in a container of $m$ memory. To emulate AWS Lambda, 
the CPU power assigned to the container is proportional to its memory based on 
the observation in \cite{xxx}. In the experiment, we adjust $m$ to 128, 256, 512, 1,024, and 2,048\,MB, 
and invoke the function with and without \sysname running. 
The guard is initialized with a local flow graph that has one path with one node, but 
the guard checks the single node 1000 times to emulate the worst case policy lookup time 
of a 1000-node graph.


We use the difference of request completion times without (i.e., using stock gVisor) 
and with \sysname to estimate the guard-checking overhead. 
As expected, guard-checking overhead increases as function memory decreases.  
When compared with using stock gVisor, the average guard-call overhead across all calls 
is 21.8\,ms~(13\%) when $m$ = 128\,MB, and only 0.7\,ms~(8\%) when $m$ = 2,048\,MB. 


\bheading{End-to-end latency of DeathStarBench applications.}
%
To understated the potential performance impact of \sysname on realistic applications, 
we further run the DeathStarBench benchmark suite~\cite{xxx} with \sysname in the local testbed, 
DeathStarBench provides a set of microservice applications, a workload generator \emph{wrk2} for generating predefined workloads for different 
applications, and a trace analysis tool that reports various performance metrics on each function as well as the entire application. 
We measure the end-to-end latencies of two DeathStarBench under various workloads: 
\begin{newitemize}
	\item social-network: The application implements a social network with unidirectional follow relationships between users. The implementation consists of loosely coupled long-running functions communicating with each other via Thrift RPC. 
	The built-in workloads for social-network are:
	\begin{itemize}
		\item compose-post: The workload involves sending POST requests to an application entry function. The data is text only with the size varying within 1KB. The request is to post the payload text on a specific user's timeline.
		\item read-home-timeline: The workload sends GET requests to an application entry function. The size of the GET requests are within 100 bytes. 
		\item read-user-timeline: This workload is similar to the read-home-timeline workload, but the requests are sent to a different entry function.
	\end{itemize}
	\item media-microsvc: The application is a movie review service where users can sign up and post reviews about movies. Similar to social-network, media-microsvc also uses Thrift RPC to communicate between different functions.
	The only provided workload for media-microsvc is:
	\begin{itemize}
		\item compose-review: The workload involves sending POST requests containing a movie review. The size of each request is within 500 bytes.
	\end{itemize}
\end{newitemize}

We run the flow tracking function in the guard. The policy generated for social-network 
has 253 nodes and 75 edges, while the policy for media-microsvc has a total of 210 nodes 
and 98 edges. We do not use the DeathStarBench applications to evaluate the efficiency 
of the flow tracking function because these application do not exhibit typical 
serverless behaviors, which may cause \sysname fail to generate accurate policies. 
For instance, a long-running function in social-network keeps listening for requests 
from other functions after being launched, and is able to generate arbitrary numbers 
of flows without exiting. However, the generated 
flow graphs only allow explicit numbers of flows from the function to prevent DoS attacks, 
and thus may incorrectly block flows from the function. Nevertheless, 
the DeathStarBench applications are developed based on realistic services, making 
them suitable for performance benchmarking.  


We run each workload \liangw{x} times and report the end-to-end latency of 




\begin{table}[t]
\footnotesize
\centering
\renewcommand\tabcolsep{1.5pt}
\begin{tabular}{|l|l|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{\textbf{Apps}} & \multicolumn{1}{c|}{\textbf{Workloads}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}\# Covered \\ Func\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}\sysname \\ Lat. (ms)\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}gVisor \\ Lat. (ms)\end{tabular}}} & \multicolumn{1}{c|}{\textbf{Overhead (\%)}} \\ \hline
\multirow{3}{*}{social} & compose-post & 10 & 26.92 & 25.86 & 4.07 \\ \cline{2-6} 
 & read-home-timeline & 1 & 8.63 & 8.38 & 2.89 \\ \cline{2-6} 
 & read-user-timeline & 1 & 8.74 & 8.38 & 4.20 \\ \hline
media & compose-review & 10 & 23.14 & 21.90 & 5.60 \\ \hline
\end{tabular}
\caption{The average end-to-end latencies of two DeathStarBench applications under different workloads, with and without \sysname.}
\label{tab:deathstar}
\end{table}


% \begin{table}[t]
% \footnotesize
% \centering
% \renewcommand\tabcolsep{1.5pt}
% \begin{tabular}{|l|l|l|l|l|l|l|}
% \hline
% \multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Apps}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Workloads}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}\#Covered \\ Functions\end{tabular}}}} & \multirow{2}{*}{\textbf{\#Events}} & \multicolumn{3}{c|}{\textbf{Policy}} \\ \cline{5-7} 
% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{\textbf{size (MB)}} & \multicolumn{1}{c|}{\textbf{\#node}} & \multicolumn{1}{c|}{\textbf{\#edges}} \\ \hline
% \hline
% \multirow{4}{*}{social} & compose-post & XXX &  &  &  &  \\ \cline{2-7} 
%  & read-home-timeline & XXX &  &  &  &  \\ \cline{2-7} 
%  & read-user-timeline & XXX &  &  &  &  \\ \cline{2-7} 
%  & \textbf{Total} & XXX & 23,944 & 2.9 & 253 & 75 \\ \hline
% media & compose-review & XXX & 38,733 & 3.9 & 210 & 98 \\ \hline
% \end{tabular}
% \caption{\liangw{finish this table}}
% \end{table}


\iffalse

\subsection{Setup}
We tested Seclambda on the DeathStarBench[cite] benchmark suite of serverless applications. We ran all our tests on a 5 machine, single control plane Kubernetes cluster, with each node running on Intel(R) Xeon(R) CPU E5-2640 v4 @ 2.40GHz and 64GB of RAM. Each machine is connected to a star topology LAN network with a speed of 25Gbps. %The network plugin used in the Kubernetes nodes was Cilium v1.6~\liangw{what is network plugin, is it important?}. 
The workloads being used were generated using the $wrk2$ workload generator provided with DeathStar bench. $wrk2$ gives a breakdown of the end to end latency of each workload as well as the distribution of the latency. The individual microservice running times are collected by analyzing traces from DeathStar's Jaeger trace collection microservice. \liangw{add a short high level description of the workload. request sizes? http GET or POST with payload?}. We use a setting of 1 request/second over 1 thread and 1 connection for 100 seconds as the test setting, because we believe that the worst case overhead is prominent at light loads. For each tested application, the guard policy was generated by collecting the runtime traces of the network system calls (SendMsg and Write) for each microservice individually. The seclambda controller runs on a separate identical node outside the LAN but on the same datacenter. \liangw{where's the controller? on one of the five machines or a separate machine?}. \liangw{more details on the policy. policy size? how many nodes? }



Specifically the applications that we tested were \liangw{can you add a flow graph like fig 4?}:
\begin{itemize}
	\item social-network : The application implements a social network with unidirectional follow relationships between users. The implementation consists of loosely coupled long running microservices communicating with each other via Thrift RPC. The policy used for social-network is 2.9MB in size and has 253 nodes, 75 edges and 23944 unique events.
	The $wrk2$ workloads for social-network are:
	\begin{itemize}
		\item compose-post : The workload involves sending POST requests to an application endpoint. The data is text only with the size varying well within 1KB. The request is to post the payload text on a specific user's timeline.
		\item read-home-timeline : The workload involves a GET request at an application endpoint. The size of the GET requests are within 100 bytes. 
		\item read-user-timeline : Similar to read-home-timeline but at a different endpoint and the size of the GET requests are within 100 bytes.
	\end{itemize}
	\item media-microsvc : The application is a movie review service where users can sign up and post reviews about movies. Similar to social-network, media-microsvc also uses Thrift RPC to communicate between the various microservices. The policy used was 3.9MB in size and had a total of 210 nodes, 98 edges and 38733 unique events.
	The $wrk2$ workloads for media-microsvc are:
	\begin{itemize}
		\item compose-review : The workload involves sending POST requests containing a movie review. The size of each request is within 500 bytes.
	\end{itemize}
\end{itemize}


\begin{table}[t]
\footnotesize
\centering
\renewcommand\tabcolsep{1.5pt}
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Apps}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Workloads}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}\#Covered \\ Functions\end{tabular}}}} & \multirow{2}{*}{\textbf{\#Events}} & \multicolumn{3}{c|}{\textbf{Policy}} \\ \cline{5-7} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{\textbf{size (MB)}} & \multicolumn{1}{c|}{\textbf{\#node}} & \multicolumn{1}{c|}{\textbf{\#edges}} \\ \hline
\hline
\multirow{4}{*}{social} & compose-post & XXX &  &  &  &  \\ \cline{2-7} 
 & read-home-timeline & XXX &  &  &  &  \\ \cline{2-7} 
 & read-user-timeline & XXX &  &  &  &  \\ \cline{2-7} 
 & \textbf{Total} & XXX & 23,944 & 2.9 & 253 & 75 \\ \hline
media & compose-review & XXX & 38,733 & 3.9 & 210 & 98 \\ \hline
\end{tabular}
\caption{\liangw{finish this table}}
\end{table}




\subsection{Performance}
\bheading{metrics.} \liangw{define the performance metrics you used how to collect them. see SecVIII Sec C}
The various performance metrics that we collected were:
\begin{itemize}
	\item End to End Application Latency: We measure the end to end application latency for the applications in DeathStar bench for various workloads when run with Seclambda and with stock gVisor. We use the $wrk2$ workload generator to generate a latency distribution for each workload as well as the average latency
	\item Microservice Runtime: We measure and compare the time taken by each microservice in a workload when run with Seclambda and with stock gVisor. DeathStar bench provides tracing of individual microservices available via a Jaeger microservice API. We used this API to collect the individual function runtimes
	
\end{itemize}

\bheading{Various overheads.}
\liangw{something like SecVIII Sec C. we really need per-system call overhead.}
\begin{itemize}
	\item Per System Call Overhead: We measure the overhead per system call of the SendMsg and Write system calls for two cases:
	\begin{itemize}
		\item Local Function Graph Lookups: We measure the time taken to check the local policy graph for a particular outgoing request when the guard does not need to contact the controller for a decision
		\item Global Function Graph Lookups: We measure the time taken to check the global policy graph residing at the controller when checking the local policy graph is insufficient for a decision
	\end{itemize}
\end{itemize}


\subsection{Security}
\liangw{using some requests to build the policy and enforce the policy against more requests to see if any false alarms. you don't need to block the requests, simply log the decisions made by the guard.}

\fi

==> main_old.tex <==
% TEMPLATE for Usenix papers, specifically to meet requirements of
%  USENIX '05
% originally a template for producing IEEE-format articles using LaTeX.
%   written by Matthew Ward, CS Department, Worcester Polytechnic Institute.
% adapted by David Beazley for his excellent SWIG paper in Proceedings,
%   Tcl 96
% turned into a smartass generic template by De Clarke, with thanks to
%   both the above pioneers
% use at your own risk.  Complaints to /dev/null.
% make it two column with no page numbering, default is 10 point

% Munged by Fred Douglis <douglis@research.att.com> 10/97 to separate
% the .sty file from the LaTeX source template, so that people can
% more easily include the .sty file into an existing document.  Also
% changed to more closely follow the style guidelines as represented
% by the Word sample file. 

% Note that since 2010, USENIX does not require endnotes. If you want
% foot of page notes, don't include the endnotes package in the 
% usepackage command, below.

% This version uses the latex2e styles, not the very ancient 2.09 stuff.

\def\showcomments{1}
\input{defs}

% \hypersetup{draft}
\begin{document}

%don't want date printed
\date{}

%make title bold and 14 pt font (Latex default is non-bold, 16 pt)
\title{\Large \bf SecLambda: Securing Serverless with Distributed Reference Monitors}

%for single author (just remove % characters)

% \author{
% {\rm Liang Wang}\\
% UW-Madison
% \and
% {\rm Mengyuan Li}\\
% Ohio State University
% \and
% {\rm Yinqian Zhang}\\
% Ohio State University
% \and
% {\rm Thomas Ristenpart}\\
% Cornell Tech
% \and
% {\rm Michael Swift}\\
% UW-Madison
% }
\makeatletter
\renewcommand\AB@affilsepx{, \protect\Affilfont}
\makeatother
\renewcommand\Authsep{, }
\renewcommand\Authands{, }

\author{}
% \author[1]{Liang Wang}
% \affil[1]{UW-Madison}

% \author[1]{Thomas Ristenpart}
% \affil[2]{Cornell Tech}

% \author[1]{Michael Swift}
% \affil[1]{UW-Madison}

% copy the following lines to add more authors
% \and
% {\rm Name}\\
%Name Institution
% } % end author

\maketitle

% Use the following at camera-ready time to suppress page numbers.
% Comment it out when you first submit the paper for review.
% \thispagestyle{empty}


\input{abstract}

\input{intro}

% \input{background}

\input{motivation}

\input{threat}

\input{design}

\input{app}

% \input{security}
\input{eval}

\input{conclusion}
% \input{aws}

% \input{gcf}

% \input{azure}

{\footnotesize \bibliographystyle{acm}
\bibliography{biblio}}


\end{document}









==> related.tex <==
% \section{Related Work}

% \bheading{AWS X-Ray.}
% %


% \bheading{AWS WAF.}
% % 
  


==> security.tex <==
\section{Security Analysis}




==> tracing_summary.tex <==
\begin{table*}[t]
\scriptsize
\def\arraystretch{1}
\begin{tabular}{|l|p{6cm}|r|r|r|r|r|}
\hline
 & \multicolumn{1}{c|}{Method} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}App\\ transparency\end{tabular}} & \multicolumn{1}{c|}{Granularity} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Cross\\ infrastructure\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Policy support\\ (w/ enforcement)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Deployment \\ difficulty\end{tabular}} \\ \hline
Xtrace~\cite{xtrace} & Runtime instrumentation; Use specialized software stack to support metadata propagation & No & High (Resource) & No & No & High \\ \hline
DVM~\cite{dvm} & Runtime instrumentation; Use Java binary rewriting to add trace points & Yes & High & No & Yes & Median \\ \hline
Pivot~\cite{pivot} & Runtime instrumentation; Use Java binary rewriting to add trace points (dynamically) & Yes & High & No & No & Median \\ \hline
\begin{tabular}[c]{@{}l@{}}Magpie~\cite{magpie} \\ Dapper~\cite{dapper}\\ Lowgo~\cite{lowgo}\end{tabular} & Runtime instrumentation; Modify libs & Yes & High & No & No & Median \\ \hline
Pinpoint~\cite{pinpoint} & Runtime instrumentation; Modify libs to propagate request ID + packet capture to get HTTP content & Yes & Median (Request) & No & No & Median \\ \hline
\begin{tabular}[c]{@{}l@{}}Pip~\cite{pip}, \\ Kronos~\cite{kronos}\end{tabular} & Program instrumentation; Modify libs & No & High & No & Yes & Median \\ \hline
FlowTags~\cite{flowtags} & Middlebox instrumentation; Modify middleboxes to propagate tags & Yes & Low (IP + port) & No & Yes & Low \\ \hline
\begin{tabular}[c]{@{}l@{}}Aguilera et al.~\cite{blackbox} \\ Orion~\cite{orion}\end{tabular} & Blackbox; Passive traffic analysis + heuristics & Yes & Low (IP + port) & Yes & - & Low \\ \hline

\end{tabular}
\caption{A comparison of methodologies for discovering application dependency.}
\end{table*}

